RefBERT: A Two-Stage Pre-trained Framework for Automatic Rename Refactoring

Refactoring is an indispensable practice of improving the quality and maintainability of source code in software evolution. Rename refactoring is the most frequently performed refactoring that suggests a new name for an identifier to enhance readability when the identifier is poorly named. However, most existing works only identify renaming activities between two versions of source code, while few works express concern about how to suggest a new name. In this paper, we study automatic rename refactoring on variable names, which is considered more challenging than other rename refactoring activities. We first point out the connections between rename refactoring and various prevalent learning paradigms and the difference between rename refactoring and general text generation in natural language processing. Based on our observations, we propose RefBERT, a two-stage pre-trained framework for rename refactoring on variable names. RefBERT first predicts the number of sub-tokens in the new name and then generates sub-tokens accordingly. Several techniques, including constrained masked language modeling, contrastive learning, and the bag-of-tokens loss, are incorporated into RefBERT to tailor it for automatic rename refactoring on variable names. Through extensive experiments on our constructed refactoring datasets, we show that the generated variable names of RefBERT are more accurate and meaningful than those produced by the existing method.

==> casestudy.tex <==




In Figure \ref{fig:casestudy}, we provide \red{six} case studies to further illustrate that the effectiveness of BoT loss on predicting masked variable names. 
\red{We observe that, if results using BoT are of low quality, results using \mathcal{L}_{\text{cMLM}} only are also of inferior quality. Hence, we selected these six cases, where \ours produces consistent results as ground truth, in three categories (more meaningful, abbreviated, and non-repetitive). }
We can see our BoT model can generate more accurate variable names. Especially, we find that our model can produce more meaningful tokens according to the context, as shown in Example 2, where “count” and “size” are synonymous to some extent. We also notice that our model can generate the stem word (e.g., “Dir” of  “Directory” in Example 1, “repr” of “Representation” in Example 4), partly because our BoT loss tends to make the generated sub-tokens semantically aligned with the code snippets. Apart from that, our model can avoid generating duplicate stem words or words(e.g., “embededsThumbnail” in Example 5, “fieldFieldValue” in Example 6), because BoT promotes the generation of bag of tokens in variables, and it is rare for a variable to contain repeated sub-tokens.

\begin{figure}[htbp]
% \label{fig:length}
    \centering
    \includegraphics[width=5in]{figs/casestudy1.pdf}
%\caption{fig1}
    \caption{Six examples of variable names generated by BoT and CE loss. The masked variables are highlighted in yellow.}
    \label{fig:casestudy}
\end{figure}
